Model Predictive Control-Based Battery Scheduling and Incentives to Manipulate Demand Response Baselines

We study operations of a battery energy storage system under a baseline-based demand response (DR) program with an uncertain schedule of DR events. Baseline-based DR programs may provide undesired incentives to inflate baseline consumption in non-event days, in order to increase "apparent" DR reduction in event days and secure higher DR payments. Our goal is to identify and quantify such incentives. To understand customer decisions, we formulate the problem of determining hourly battery charging and discharge schedules to minimize expected net costs, defined as energy purchase costs minus energy export rebates and DR payments, over a sufficiently long time horizon (e.g., a year). The complexity of this stochastic optimization problem grows exponentially with the time horizon considered. To obtain computationally tractable solutions, we propose using multistage model predictive control with scenario sampling. Numerical results indicate that our solutions are near optimal (e.g., within 3% from the optimum in the test cases). Finally, we apply our solutions to study an example residential customer with solar photovoltaic and battery systems participating in a typical existing baseline-based DR program. Results reveal that over 66% of the average apparent load reduction during DR events could result from inflation of baseline consumption during non-event days.

==> model_Aug6.tex <==
\section{MODEL} \label{MODEL}
\subsection{Problem Formulation}
We consider a customer with electric loads, a solar photovoltaic system, and a battery energy storage system. The customer participates in a baseline-based demand response program and is subject to a certain electricity tariff. Our objective is to determine the optimal schedule of battery charging and discharging to minimize expected net costs for the customer over a series of days $t \in \{1,\ldots,t_{final}\}$. 

The goal of the demand response program is to incentivize the customer to reduce electricity consumption during a pre-specified window of hours (e.g., 5 p.m -- 9 p.m.) on certain demand response \textit{event days}. The customer is notified whether the current day is an event day at the beginning of each day. For days after the current day, we assume that the customer knows the probability that each day will be an event day (e.g., the probability of event may be correlated with the weather).

In each hour $h \in \{1,\ldots,(24 \cdot t_{final}) \}$, the customer has a given default electricity demand $d_h$ and a given solar energy production $s_h$. [[note -- in practice these are not know in advance...these uncertainties are beyond the scope of this paper. ]] Also in each hour, the customer can decide to charge the battery $b^+_h$ or discharge the battery $b^-_h$, resulting in an hourly net load $l_h = d_h + b^+_h - s_h - b^-_h$. The default electricity demand $d_h$ and solar production $s_h$ are model parameters, and battery charging $b^+_h$ and discharging $b^-_h$ are decision variables. Positive values of $l_h$ indicate that the customer purchases energy from the grid during hour $h$, and negative values indicate that the customer exports energy to the grid. The values $d_h$, $s_h$, $b_h$, and $l_h$ are in units of kW or kWh (since the time-step is one hour, the kW and kWh quantities are equivalent).

The battery decision variables, $b^+_h$ and $b^-_h$, can take on non-negative real values, and are restricted by constraints that represent the physical characteristics of a battery energy storage system. A power capacity constraint requires that $b^+_h + b^-_h$ less than the rated power capacity of the battery system for all hours. An energy capacity constraint requires that the level of energy stored in the battery is always greater than or equal to zero and less than or equal to the rated energy capacity of the battery system. The level of stored energy is calculated as the level of stored energy in the prior hour plus $b^+_h \cdot \eta^+$ minus $b^-_h / \eta^-$, where $\eta^+$ is battery charging efficiency and $\eta^-$ is battery discharging efficiency.

Part of the customer's net costs are determined by the customer's electricity tariff. For each hour when $l_h \ge 0$, the customer incurs an energy purchase cost, $c^{kWh}_h$, calculated as
\begin{eqnarray} \label{eqn:ckwh}
c^{kWh}_h = r^{c,kWh}_h \cdot l_h,
\end{eqnarray}
where $r^{c,kWh}_h$ is the \$/kWh electricity purchase rate for hour $h$. For each hour when $l_h < 0$, the customer receives an energy export payment, $p^{kWh}_h$, calculated as
\begin{eqnarray} \label{eqn:pkwh}
p^{kWh}_h = r^{p,kWh}_h \cdot (-l_h),
\end{eqnarray}
where $r^{p,kWh}_h$ is the \$/kWh electricity export rate for hour $h$. Hourly electricity purchase and export rates are model parameters, which can be determined by the customer tariff. 

Additionally, the customer may receive DR energy payments ($p^{DR,kWh}_t$) or DR power payments ($p^{DR,kW}_i$) or both via the demand response program. Both types of DR payments are based on the quantity of demand response energy reduction, $q^{DR,kWh}_t$, for each day $t$ that is an event day, which is calculated by
\begin{eqnarray} \label{eqn:qdr}
q^{DR,kWh}_t = (e^{BL}_t - e^{DR}_t),
\end{eqnarray}
where $e^{BL}_t$ is the baseline energy consumption for day $t$ and $e^{DR}_t$ is the energy consumption during the DR window for day $t$. DR window energy consumption is calculated by
\begin{eqnarray}
e^{DR}_t = \sum_{h \in H^{DR}_t}{l_h},
\end{eqnarray}
where $H^{DR}_t$ denotes the set of hours corresponding to the DR window for day $t$. Baseline energy consumption is calculated by some function of the demand response window energy consumption of $N_B$ preceding non-event days (e.g., the average DR window energy consumption over 10 preceding non-event days). [[Note that some programs distinguish weekday/weekend.]]

Given $q^{DR,kWh}_t$, the DR energy payments $p^{DR,kWh}_t$ for each event day $t$ is calculated by
\begin{eqnarray} \label{eqn:pdrkwh}
p^{DR,kWh}_t = r^{DR,kWh}_t \cdot q^{DR,kWh}_t,
\end{eqnarray}
where $r^{DR,kWh}_t$ is the \$/kWh DR payment rate for day $t$. The customer receives no DR energy payments on non-event days. 

A DR capacity payment is made for each interval $i$, which may correspond, for example, to each month. The DR capacity payment for interval $i$ is calculated by the DR capacity payment rate multiplied by the average kW load reduction over all DR event hours in interval $i$, or
\begin{eqnarray} \label{eqn:pdrkw}
p^{DR,kW}_i = r^{DR,kW}_i \cdot \frac{\displaystyle \sum_{t \in T^{DR}_i}{q^{DR,kWh}_t}}{\displaystyle \sum_{t \in T^{DR}_i} |H^{DR}_t|},
\end{eqnarray}
where $r^{DR,kW}_i$ is the DR capacity payment rate for interval $i$, and $T^{DR}_i$ is the set of DR event days in interval $i$. [[Discuss how to deal with no DR events...We include 0, other programs do give credit...]]

The customer's total cost for a given realization of which days are event days is calculated as 
\begin{eqnarray} \label{eqn:customercost}
c = \sum_{h}{[c^{kWh}_h - p^{kWh}_h]} - \sum_{t}{p^{DR,kWh}_t} - \sum_i{p^{DR,kW}_i},
\end{eqnarray}
and the customer's objective is to minimize the expectation of $c$ over all possible realizations of events days. 

\subsection{Model Predictive Control Approach}
The customer's problem is a multi-stage stochastic decision problem, with $2^{t_{final}}$ stochastic scenarios, corresponding to all possible unique assignments of each day to event day or non-event day. For small values of $t_{final}$, this can be formulated and solved as a single stochastic program, but for larger values of $t_{final}$, the complete problem becomes too large and approximate solution methods are required. For example, if we consider a timeframe of one year, $t_{final}$ is 365 and the full problem has over $10^{111}$ unique decision variables. 

We obtain a near-optimal solution to this problem using a multistage model predictive control approach, with a receding horizon of $n$ days. For each day, we solve a stochastic program representing the customer's decisions and costs over the next $n$ days, where $n \leq t_{final}$. We save and use the decisions for the current day, and repeat this process for each day. The hypothesis behind this approach is that when $n$ is sufficiently large, there is a small chance of the current day's action having a significant impact on costs more than $n$ days in the future, so the current day customer decisions for this smaller stochastic program are likely to be close to the optimal current day decisions. [[discuss this in more detail. normally this comes from discounting, but for us it comes from the structure of the problem.]]

The stochastic linear program over that is solved for each day was implemented using Pyomo \cite{article}\cite{HartWilliamE.2017P—OM} and PySP \cite{WatsonJean-Paul2012Pmas}. The stochastic program is formulated as a linear program in Pyomo that represents decisions, constraints, and costs for a single realization of stochastic parameters (i.e. a single scenario), and a PySP scenario tree that determines non-anticipativity constraints for decisions of various scenarios and how to weight scenario costs in the expected value calculation. The following sections describe the linear program for a single scenario and the scenario tree. 

\subsection{Scenario Tree Structure}
The relationship between the various scenarios (representing different possible realizations of event days) are defined in the scenario tree. The tree structure is created based on the parameters $n$, the number of days in the model predictive control horizon, and $n_{tree} \leq n$, where the total number of scenarios included is $2^{n_{tree}}$. For the first $n_{tree}$ days of the horizon, the scenario tree includes the full tree, with branches representing both event and no event each day. For the remaining $n - n_{tree}$ days in the horizon, each scenario includes just one sample event schedule, where the occurrence of an event on day $t \in \{ n_{tree}+1, ... ,n \}$ sampled randomly for each scenario with probability $\mathbb{P}_t$, the probability day $t$ is an event day. If $n$ or $n_{tree}$ days from the current day extends past $t_{final}$, only the remaining days through $t_{final}$ are included in the scenario tree. 

Each scenario has associated parameters, decisions, constraints, and cost as described in the next section. The scenario tree imposes non-anticipativity constraints that require scenarios with identical event schedules for days $1,...,t$ must also have identical decision variable values for those days. 

The objective of the stochastic program is to minimize the expectation of the cost over the scenarios, where the probability of each scenario is calculated by $\prod_{t \in \{ 1, ..., n_{tree} \}}{\mathbb{P}_t}$. When the current horizon of $n$ days runs through $t_{final}$ and $n_{tree} = n$, the objective function represents the true expected future customer cost. However, when $n$ and $n_{tree}$ are smaller, this objective serves as an approximation of the true cost. The approximation may differ from the true cost due to not calculating costs through the end of the period, not calculating costs for all possible scenarios, and not including non-anticipativity constraints for days after $n_{tree}$. The required minimum values for $n$ and $n_{tree}$ to yield a suitable approximation for determining current day near-optimal actions are case-specific. Numerical results in section [TBD] illustrate the success of this approximation in some small example cases, where we can compare the approximate solutions to the true optimal solution. For larger problems, $n$ and $n_{tree}$ can be set based on available computational resources, in order to obtain a feasible and potentially near-optimal set of decisions, but without guarantee of closeness to optimality.  

\subsection{Single Scenario Linear Program Formulation}
The single scenario linear program formulation describes the parameters, decisions variables, constraints, and costs for a single realization of the stochastic parameters (i.e., a specification of which days are event days) over the next $n$ days.

\paragraph{Parameters}
The model parameters that distinguish the various scenarios within the stochastic program are the specification of which days are event days. Each scenario in the stochastic program has a different set of days that are event days. 

The other model parameters are the same for all scenarios within the stochastic program. Calendar-related parameters include specification of which days are in which DR capacity payment interval, and the total number of days in each interval. Model parameters relating to the customer include the hourly electricity demand $d_h$, the hourly solar production $s_h$, and the capabilities of the customer battery system (power capacity $b_{max}$, energy capacity $SOC_{max}$, and efficiencies $\eta_+$ and $\eta_-$). The customer tariff determines the hourly grid energy cost rate $r_h^{c,kWh}$ and export rebate rate $r_h^{p,kWh}$. The demand response program design determines which hours of the day are the DR window $H_t^{DR}$ (i.e. the hours that determine event load event days and baseline load on non-event days), the number of days in the DR baseline $N_B$, and the DR energy and capacity payment rates $r_t^{DR,kWh}$ and $r_i^{DR,kW}$. Some parameters are set based on what occurred prior to the current horizon: the initial customer baseline, which is a series of $N_B$ values of DR window energy consumption on prior non-event days, the battery's initial state of charge $SOC_0$, the number of prior event hours that have occurred in the current interval $|H_0^{DR}|$, and the load reduction in those prior events $q_0^{DR,kWh}$. 

\paragraph{Decision variables}
The decision variables are the hourly quantities of battery charging $b_h^+$ and discharging $b_h^-$. 

\paragraph{Constraints}
The battery decision variables, $b^+_h$ and $b^-_h$, can take on non-negative real values, and are restricted by constraints that represent the physical characteristics of a battery energy storage system. A power capacity constraint requires that $b^+_h + b^-_h$ less than the rated power capacity of the battery system for all hours. An energy capacity constraint requires that the level of energy stored in the battery is always greater than or equal to zero and less than or equal to the rated energy capacity of the battery system. The level of stored energy is calculated as the level of stored energy in the prior hour plus $b^+_h \cdot \eta^+$ minus $b^-_h / \eta^-$, where $\eta^+$ is battery charging efficiency and $\eta^-$ is battery discharging efficiency.

\paragraph{Cost function}
The cost in each scenario contribute to the objective function for the stochastic program, which is the expectation of cost over all scenarios. The scenario cost is an estimate of net costs associated with the $n$ day horizon, where positive costs are energy purchases from the grid $c_h^{kWh}$, and negative costs (i.e., payments) are rebates from exports to the grid $p_h^{kWh}$, DR energy payments $p_t^{DR,kWh}$, and DR capacity payments $p_i^{DR,kWh}$. 
The cost components $c_h^{kWh}$, $p_h^{kWh}$, and $p_t^{DR,kWh}$ are calculated for the hours and days in the current model predictive control horizon of $n$ days according to \eqref{eqn:ckwh}, \eqref{eqn:pkwh}, and \eqref{eqn:pdrkwh}. For intervals that are entirely included in the current horizon, $p_i^{DR,kWh}$ is calculated according to \eqref{eqn:pdrkw}. If the first interval in the current horizon had prior events before the horizon, the prior event parameters are used to calculate $p^{DR,kW}_i$ for the entire interval as
\begin{eqnarray} \label{eqn:pdrkwfirst}
p^{DR,kW}_i = r^{DR,kW}_i \cdot \frac{q_0^{DR,kWh} + \displaystyle \sum_{t \in T^{DR}_i}{q^{DR,kWh}_t}}{|H_0^{DR}| + \displaystyle \sum_{t \in T^{DR}_i} |H^{DR}_t|}.
\end{eqnarray}
If the last interval in the current horizon ends after the end of the horizon, $p_i^{DR,kWh}$ for that interval is first calculated according to \eqref{eqn:pdrkw} over that interval's days in the horizon, and then it is multiplied by the fraction of total days in the interval that are included in the horizon. This portion of the last interval's DR capacity payment is included to align with the portion of the month for which tariff costs and DR energy payments are included. 

==> results.tex <==
\section{RESULTS}

\subsection{}

\begin{table}
  \caption{Approximation study results: Jan. 1-7}
  \label{table:1}
  \includegraphics[width=\linewidth]{jan7dayapprox.png}
\end{table}

\begin{table}
  \caption{Approximation study results: Oct. 1-7}
  \label{table:2}
  \includegraphics[width=\linewidth]{oct7dayapprox.png}
\end{table}

\begin{table}
  \caption{Full-year results: no DR payment}
  \label{table:3}
  \centering
  \includegraphics{fullyearnodr.png}
\end{table}

\begin{table}
  \caption{Full-year results: \$2/kW-month DR capacity payment}
  \label{table:4}
  \centering
  \includegraphics{fullyeardr2.png}
\end{table}

\begin{table}
  \caption{Full-year results: \$10/kW-month DR capacity payment}
  \label{table:5}
  \centering
  \includegraphics{fullyeardr10.png}
\end{table}




\iffalse

The stochastic linear programs described in section \ref{CASE STUDY} were solved in order to obtain hourly battery dispatches for each case, month, and scenario. Then, the hourly battery dispatches were used to calculate the expected values of various metrics for each case and month. These metrics are presented in figure \ref{fig:allresults}. The DR quantity and cost metrics for all cases are calculated as if the customer were participating in the standard Capacity Reduction DR program. While different cost models were used in the optimizations for each case, using the standard Capacity Reduction cost model to calculate result metrics facilitates comparisons between cases. 

The metrics included in figure \ref{fig:allresults} are described below:
DR events is the expected number of DR events that occur in the calendar month.
Baseline is the expected value of the customer baseline energy consumption, $e^{BL}_t$, over all event days.
DR is the expected value of average monthly kW load reduction. This reflects the difference between baseline energy consumption and event energy consumption.
Tariff cost is the expected value of customer energy purchase costs minus customer energy export payments. Minimizing tariff costs is the objective of Case 3, because DR payments are not considered in the optimization for that case.
DR payment is the expected value of DR monthly capacity payments.
Customer cost is  the expected value of customer cost, which is tariff cost minus DR payment. 
\begin{figure}
  \includegraphics[width=\linewidth]{allresults.png}
  \caption{Expected values of various metrics for each month and model type.}
  \label{fig:allresults}
\end{figure}

Figure \ref{fig:monthlyvals} provides a condensed summary of these metrics, with average monthly expected values for each of the three cases. Several observations can be made based on these summary metrics. 

First we see that the average DR quantity in Case 3 is approximately zero, as we would expect since Case 3 was optimized based on the assumption of no DR payments. The monthly DR values for Case 3 may be positive or negative, representing essentially random differences between baseline and event load that tend to cancel out over time. 

Alternatively, Case 2 and Case 1 both include positive average DR quantities of 1.5 kW and 1.9 kW, respectively. This indicates that even at the minimum payment level, the Capacity Reduction grid service does successfully provide an incentive for the customer to modify battery charging to deliver DR. Comparing the quantity of average DR (1.5 to 1.9 kW) to the size of the battery system (10 kW, 27 kWh), we see that the quantity of DR is much smaller than what could be obtained if the battery was solely focused on delivering DR. This makes sense, because the battery is also being used for the high-value application of shifting excess solar production to reduce tariff costs. We see that the quantity of DR varies from month to month, which likely reflects in part how much the battery is occupied by solar energy shifting. 

Next, we see that average baseline load in Case 1 (1.0 kW) is significantly higher than average baseline load in Cases 2 and 3 (0.6 kW). This 0.4 kW of average increase in baseline load is evidence of the incentive to increase baseline load in the Capacity Reduction DR program. We also see that this 0.4 kW increase in baseline load is equal to the 0.4 kW increase in DR quantity between Cases 1 and 2. This indicated that the higher DR quantity for Case 1 may be entirely due to inflated baseline load, as opposed to any additional demand reduction during events. 

Furthermore, the fact Scenario 2 has a higher DR quantity and nearly equal baseline load compared to Scenario 3 shows that it is possible to create incentives to respond to DR events without creating a significant increase in baseline load.

\begin{figure}
  \includegraphics[width=\linewidth]{monthlyvals.png}
  \caption{Average of monthly expected values of various metrics for each model type.}
  \label{fig:monthlyvals}
\end{figure}

The baseline inflation effect is further demonstrated in figure \ref{fig:blinflation}, which shows the level of baseline inflation in Case 1 in terms of kW and as a percentage of the Case 1 DR quantity for each month. Figure \ref{fig:blinflation} shows that the quantity and percentage of baseline inflation varies significantly from month to month. Compared to Case 3 (no DR), the maximum monthly baseline inflation is 1.5 kW in December, which represents 39\% of that month's apparent DR quantity. Over the year, baseline inflation accounts for 22\% of the apparent DR quantity. 
\begin{figure}
  \includegraphics[width=\linewidth]{blinflation.png}
  \caption{Baseline inflation in Case 1 compared to Cases 2 and 3.}
  \label{fig:blinflation}
\end{figure}

The differences in the results for each case are the result of different dispatch patterns for the battery. It is difficult to visualize the differences in the dispatch across all of the cases, months, scenarios, days, and hours, but figure \ref{fig:dispatch} demonstrates the hourly dispatch for the three cases for the first week in October for a single scenario. The scenario shown includes DR event days on days 3 and 4 of the week. The DR windows of 5 p.m. - 9 p.m. for each day are highlighted, which facilitates comparing dispatch during non-event DR windows (i.e. baseline-setting hours) and during event hours. 

\begin{figure}
  \includegraphics[width=\linewidth]{dispatch1.png}\\
  \includegraphics[width=\linewidth]{dispatch2.png}\\
  \includegraphics[width=\linewidth]{dispatch3.png}
  \caption{Hourly dispatch for the first week in October for each model type for the scenario with events on days 3 and 4.}
  \label{fig:dispatch}
\end{figure}

Focusing first on the day 3 and 4 events for this sample week, we see that the dispatches appear identical across all cases, with battery discharging covering the entire customer load. This indicates that the solar energy shifting application already results in load being eliminated for those hours, and it is not worthwhile to use the battery to export power to the grid during those hours to generate higher DR payments. 

Now looking at the non-event days 1, 2, 5, 6, and 7, we see that Cases 2 and 3 have approximately identical dispatches during DR windows, while Case 1 has greater purchases of energy from the grid on days 1, 2, 5, and 6. The greater energy purchases on those days appear to be primarily achieved by shifting grid energy purchases from other hours into those baseline-setting hours. Additionally, on day 6, the battery is charged from the grid during part of the baseline-setting window to further increase baseline load. 

In general, we can also observe that differences in battery dispatch patterns between scenarios are subtle, especially considering the variations in dispatch patterns within a scenario. This suggests that it may be difficult for a utility to identify or police baseline gaming behaviors, especially if the utility only sees the customer net load without information about battery operations. 

\fi
